DiffAtlas: GenAI-fying Atlas Segmentation via Image-Mask Diffusion

Accurate medical image segmentation is crucial for precise anatomical delineation. Deep learning models like U-Net have shown great success but depend heavily on large datasets and struggle with domain shifts, complex structures, and limited training samples. Recent studies have explored diffusion models for segmentation by iteratively refining masks. However, these methods still retain the conventional image-to-mask mapping, making them highly sensitive to input data, which hampers stability and generalization. In contrast, we introduce DiffAtlas, a novel generative framework that models both images and masks through diffusion during training, effectively ``GenAI-fying'' atlas-based segmentation. During testing, the model is guided to generate a specific target image-mask pair, from which the corresponding mask is obtained. DiffAtlas retains the robustness of the atlas paradigm while overcoming its scalability and domain-specific limitations. Extensive experiments on CT and MRI across same-domain, cross-modality, varying-domain, and different data-scale settings using the MMWHS and TotalSegmentator datasets demonstrate that our approach outperforms existing methods, particularly in limited-data and zero-shot modality segmentation. Code is available at https://github.com/M3DV/DiffAtlas.

==> tex/method_backup.tex <==
\input{fig/diffaltas_model}

\section{Method}

\subsection{Overview}
Atlas-based segmentation methods enforce anatomical consistency and global structure in segmentation masks, which are crucial for medical imaging. However, traditional approaches rely on predefined atlases and complex registration processes, leading to high computational costs and limited flexibility for diverse anatomical variations.

To address these issues, we propose DiffAtlas, a novel framework that integrates atlas priors with the flexibility of generative models. By learning a generative atlas space through a diffusion process, DiffAtlas eliminates explicit atlas registration while preserving global consistency. This enables accurate, reliable, and computationally efficient segmentation for diverse anatomical structures.

\subsection{Revisiting Previous Methods}

\subsubsection{Image-Conditional Feedforward Network}

Feedforward neural networks, such as U-Net, are widely used for image segmentation tasks. These models learn a deterministic mapping from the input image $\mathbb{I}$ to the segmentation mask $\mathbb{S}$, denoted as $f_\theta: \mathbb{I} \rightarrow \mathbb{S}$. The training objective typically minimizes the cross-entropy loss, dice loss, or their combination.

While efficient, these methods entirely rely on the input image, making them highly sensitive to input conditions such as noise, artifacts, or incomplete information. Furthermore, the lack of global anatomical priors limits their ability to enforce structural consistency, reducing robustness and generalization in complex anatomical regions or across diverse datasets.

\subsubsection{Image-Conditional Mask Diffusion}

Image-Conditional Mask Diffusion extends the image-conditional paradigm by modeling the conditional distribution $p(S|I)$, where $S$ is the segmentation mask and $I$ is the input image. By introducing a probabilistic framework, Image-Conditional Mask Diffusion decomposes the generation of the segmentation mask into a step-by-step denoising process. The forward process progressively corrupts the ground-truth mask with Gaussian noise:

\begin{equation}
q(S_t|S_{t-1}) = \mathcal{N}(S_t; \sqrt{\alpha_t} S_{t-1}, (1-\alpha_t) \mathbf{I}),
\end{equation}

while the reverse process iteratively refines the noisy mask by learning the conditional distribution $p_\theta(S_{t-1}|S_t, I)$:

\begin{equation}
p_\theta(S_{t-1}|S_t, I) = \mathcal{N}(S_{t-1}; \mu_\theta(S_t, I, t), \Sigma_\theta(S_t, I, t)).
\end{equation}

The introduction of stochasticity enables the generation of diverse plausible masks. However, these methods remain tied to the image-conditional paradigm, making them sensitive to input noise and lacking robustness and generalization.

\subsubsection{Registration-Based Atlas}

Atlas-based methods address the lack of global priors by leveraging predefined labeled atlases $(A_I, A_S)$. These methods register the atlas image $A_I$ to the target image $I$, propagating the atlas labels $A_S$ through the deformation field $\phi^*$:

\begin{equation}
S = A_S \circ \phi^*,
\end{equation}

where the deformation field $\phi^*$ is computed by minimizing an energy function:

\begin{equation}
\phi^* = \arg\min_\phi \mathcal{D}(I, A_I \circ \phi) + \lambda \mathcal{R}(\phi),
\end{equation}

with $\mathcal{D}$ measuring similarity between $I$ and the deformed atlas $A_I \circ \phi$, and $\mathcal{R}$ being a regularization term. While effective in enforcing anatomical consistency, these methods are computationally expensive and heavily depend on the quality of the predefined atlas, limiting their flexibility for diverse anatomical variations.

\subsection{DiffAtlas Framework}

\subsubsection{Joint Modeling Image-Mask Prior in a Generative Atlas Space}

DiffAtlas models the image-mask pair $(I, S)$ in a generative atlas space learned through a diffusion process. Unlike traditional atlas-based methods relying on predefined atlases, this approach captures global consistency while accommodating diverse anatomical structures. During training, DiffAtlas learns the joint distribution $p_\theta(I, S)$ by reconstructing clean pairs $(I, S)$ from noisy versions $(I_t, S_t)$, ensuring anatomically consistent and image-aligned segmentation masks.

\subsubsection{Noisy Image Guidance for Input-Conditioned Sampling}

DiffAtlas employs noisy image guidance to align segmentation masks with the input image during inference. At each timestep $t$, the noisy input image $I_t$ is updated as:

\begin{equation}
I_t = \sqrt{\alpha_t} I_\text{input} + \sqrt{1-\alpha_t} \epsilon,
\end{equation}

where $\epsilon$ is Gaussian noise. This ensures that the diffusion process is conditioned on $I_\text{input}$, yielding segmentation masks that align closely with anatomical structures while preserving global consistency.

\subsubsection{Training Process}

During training, DiffAtlas optimizes a neural network to predict the added noise $\epsilon$ in the forward diffusion process. The training objective minimizes the mean squared error between the predicted noise $\epsilon_\theta$ and the true noise $\epsilon$:

\begin{equation}
\mathcal{L}_{\text{train}} = \mathbb{E}_{(I, S), t, \epsilon} \left[\|\epsilon - \epsilon_\theta(I_t, S_t, t)\|^2\right].
\end{equation}

This objective enables the model to learn the joint distribution of image-mask pairs $(I, S)$, ensuring that the generated segmentation masks are anatomically valid and consistent with their corresponding images.

\subsubsection{Inference Process}

During inference, DiffAtlas begins with a noisy pair $(I_T, S_T)$ and iteratively denoises it over $T$ steps. At each timestep $t$, the noisy input image $I_t$ is updated using the noisy image guidance strategy. This ensures that the reverse diffusion process remains conditioned on $I_\text{input}$, yielding a clean pair $(I, S)$, where $S$ is an anatomically consistent segmentation mask aligned with $I_\text{input}$.
